Investigating the Impact of Observation Space Design Choices On Training Reinforcement Learning Solutions for Spacecraft Problems

Recent research using Reinforcement Learning (RL) to learn autonomous control for spacecraft operations has shown great success. However, a recent study showed their performance could be improved by changing the action space, i.e. control outputs, used in the learning environment. This has opened the door for finding more improvements through further changes to the environment. The work in this paper focuses on how changes to the environment's observation space can impact the training and performance of RL agents learning the spacecraft inspection task. The studies are split into two groups. The first looks at the impact of sensors that were designed to help agents learn the task. The second looks at the impact of reference frames, reorienting the agent to see the world from a different perspective. The results show the sensors are not necessary, but most of them help agents learn more optimal behavior, and that the reference frame does not have a large impact, but is best kept consistent.

==> ref_continuous.tex <==
\subsubsection{Sample Complexity}

\begin{figure}
    \centering
    \subfigure[Total Reward]{\includegraphics[width=.45\linewidth]{figures/continuous/different_reference_frame/TotalReward_sample_eff.png}} \quad
    \subfigure[Success]{\includegraphics[width=.45\linewidth]{figures/continuous/different_reference_frame/Success_sample_eff.png}} \\
    \subfigure[Inspected Points]{\includegraphics[width=.45\linewidth]{figures/continuous/different_reference_frame/InspectedPoints_sample_eff.png}} \quad
    \subfigure[DeltaV]{\includegraphics[width=.45\linewidth]{figures/continuous/different_reference_frame/DeltaV_sample_eff.png}} \\
    \subfigure[Legend for all configurations]{\includegraphics[width=.45\linewidth]{figures/continuous/different_reference_frame/legend.png}}
    \caption{The sample complexity for \todo{fill in} (the legend is the bottom left).}
    \label{fig:something_idk}
\end{figure}

\subsubsection{Final Policy Performance}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=\linewidth]{figures/continuous/different_reference_frame/TotalReward_int_est.png}} \\
    \subfigure[]{\includegraphics[width=\linewidth]{figures/continuous/different_reference_frame/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=\linewidth]{figures/continuous/different_reference_frame/InspectedPoints_int_est.png}} \\
    \subfigure[]{\includegraphics[width=\linewidth]{figures/continuous/different_reference_frame/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs.}
    \label{fig:impact_count}
\end{figure}

==> ref_discrete.tex <==
\subsubsection{Sample Complexity}

\begin{figure}
    \centering
    \subfigure[Total Reward]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/TotalReward_sample_eff.png}} \quad
    \subfigure[Success]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/Success_sample_eff.png}} \\
    \subfigure[Inspected Points]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/InspectedPoints_sample_eff.png}} \quad
    \subfigure[DeltaV]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/DeltaV_sample_eff.png}} \\
    \subfigure[Legend for all configurations]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/legend.png}}
    \caption{The sample complexity for \todo{fill in} (the legend is the bottom left).}
    \label{fig:something_idk}
\end{figure}

\subsubsection{Final Policy Performance}

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_reference_frame/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs.}
    \label{fig:impact_count}
\end{figure}








==> sensors_continuous.tex <==
\subsubsection{How Does the Count Sensor Impact Learning?}

The count sensor has mixed results both helping and hurting performance. In every case, adding the count sensor decreases the number of inspected points, but the decrease is offset by improve fuel efficiency when used with the UPS. When the count sensor is the only additional sensor used, the agent consistently learns poor behavior that performs worse (fewer inspected points using more fuel) than having no sensors at all.

Looking at the two best performing configurations, `All Sensors - Count` and `All Sensors` we can see that adding the count sensor decreases the expected number of inspected points from 98.99 (all points) to 95.85. However, the decrease in inspected points comes with a decrease in expected fuel use from 21.85 m/s to 13.04 m/s. Choosing between these 2 configurations requires considering how important inspecting the last 3-4 points is. Is it worth spending an extra ~9 m/s to inspect the final ~3 points?

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/count_effect/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/count_effect/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/count_effect/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/count_effect/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs. The top shows performance without the count sensor and the one below shows with the count sensor. This makes it easier to see the direct impact of adding the sensor.}
    \label{fig:impact_count}
\end{figure}


\subsubsection{How Does the Sun Angle Sensor Impact Learning?}

Including the Sun Angle Sensor always decreases the total Delta V usage, which leads to an increased total reward. However, this more fuel-efficient behavior comes at the cost of fewer inspected points except when used with just the UPS.

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/sun_angle_effect/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/sun_angle_effect/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/sun_angle_effect/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/sun_angle_effect/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs. The top shows performance without the count sensor and the one below shows with the count sensor. This makes it easier to see the direct impact of adding the sensor.}
    \label{fig:impact_sun_angle}
\end{figure}

When we look at the sample complexity plots, and focus on the inspected points (shown below), we see that including the sun angle sensor helps agents inspect more points early in training, but the benefit quickly collapses in favor of saving fuel. This is shown in the figure below. On the left, we have reward consistently increasing while on the right the number of inspected points starts to decrease. The top row shows all configurations and in the bottom row, we have extracted just the \textit{Sun Angle + Count} configuration to highlight the trend since it is the most drastic.

\begin{figure}
    \centering
    \subfigure[Total Reward with all sun angle configurations]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/only_sun_angle_agents/TotalReward_sample_eff.png}} \quad
    \subfigure[Inspected Points with all sun angle configurations]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/only_sun_angle_agents/InspectedPoints_sample_eff.png}} \\
    \subfigure[Total Reward only Sun Angle + Count]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/sun_angle_count/TotalReward_sample_eff.png}} \quad
    \subfigure[Inspected Points only Sun Angle + Count]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/sun_angle_count/InspectedPoints_sample_eff.png}} \\
    \subfigure[Legend for all sun angle configurations]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/only_sun_angle_agents/legend.png}}
    \caption{Top shows the sample complexity for Total Reward and Inspected Points for all configuration with the sun angle sensor (the legend is the bottom left). Bottom shows the sample complexity for just the Sun Angle + Count configuration to highlight the effect.}
    \label{fig:something_idk}
\end{figure}

This behavior points towards the outsized cost of fuel for this problem. During training, we use a reward schedule that increases the cost of fuel for agents that have learned to inspect more than 90\% of points. The cost decreases when the agents start to inspect fewer than 80\% of points. This was intended to help the agent first focus on inspecting points and then finding the most fuel efficient policy for completing inspection. In the future we should consider investigating the impact of starting training with a more fuel efficient solution (e.g. already on a natural motion trajectory) as that might help find minimal adjustments needed to still inspect all points even with a moving chief.

\subsubsection{How Does the Uninspected Points Sensor Impact Learning?}

Including the UPS always decreases the total Delta V usage and (except when added with the just the count sensor) always decreases the episode length. Unlike with the sun angle sensor, using the UPS to decrease fuel usage does not come at the cost of inspecting fewer points and increasing the episode length. Additionally, the number of points inspected increases and the majority of agents converge on policies that inspect all points. The only configurations where learned policies converge at a success rate higher than 75\% make use of the UPS. Without the UPS, agents rarely learn to inspect all the points more than 60\% of the time.

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/ups_effect/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/ups_effect/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/ups_effect/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/ups_effect/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs. The top shows performance without the count sensor and the one below shows with the count sensor. This makes it easier to see the direct impact of adding the sensor.}
    \label{fig:impact_ups}
\end{figure}

To highlight the impact of the UPS on helping agents inspect all 99 inspection points, we present the done conditions for the final policies trained with and without the UPS below. On the left are the done conditions reported for all 10 RL agents trained using a configuration without the UPS. On the right are the reported done conditions for all 10 RL agents trained using a configuration with the UPS. In both cases illustrated below, we see a large jump in the percentage of done conditions that show `SuccessfulInspection`.

\begin{figure}
    \centering
    \subfigure[AllButUPS]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/final_dones/count_sun_angle_final_policy_done.png}} \quad
    \subfigure[WithUPS]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/final_dones/baseline_final_policy_done.png}} \\
    \caption{The done conditions for all the learned policies looking at `All Sensors - UPS` on the left and `All Sensors` on the right. The increase in successful inspections from 26.7\% to 47.5\% shows more agents learning to converge to successful behavior.}
    \label{fig:impact_ups}
\end{figure}

\begin{figure}
    \centering
    \subfigure[count]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/final_dones/count_final_policy_done.png}} \quad
    \subfigure[countUPS]{\includegraphics[width=.45\linewidth]{figures/continuous/different_obs_spaces/final_dones/count_uninspected_final_policy_done.png}} \\
    \caption{The done conditions for all the learned policies looking at `Count` on the left and `Count + UPS` on the right. The increase in successful inspections from 33.4\% to 49.6\% shows more agent al learning to converge to successful behavior.}
    \label{fig:impact_ups}
\end{figure}

==> sensors_discrete.tex <==
\subsubsection{How Does the Count Sensor Impact Learning?}

% The count sensor has mixed results both helping and hurting performance. In every case, adding the count sensor decreases the number of inspected points, but the decrease is offset by improve fuel efficiency when used with the UPS. When the count sensor is the only additional sensor used, the agent consistently learns poor behavior that performs worse (fewer inspected points using more fuel) than having no sensors at all.

% Looking at the two best performing configurations, `All Sensors - Count` and `All Sensors` we can see that adding the count sensor decreases the expected number of inspected points from 98.99 (all points) to 95.85. However, the decrease in inspected points comes with a decrease in expected fuel use from 21.85 m/s to 13.04 m/s. Choosing between these 2 configurations requires considering how important inspecting the last 3-4 points is. Is it worth spending an extra ~9 m/s to inspect the final ~3 points?

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/count_effect/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/count_effect/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/count_effect/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/count_effect/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs. The top shows performance without the count sensor and the one below shows with the count sensor. This makes it easier to see the direct impact of adding the sensor.}
    \label{fig:impact_count}
\end{figure}


\subsubsection{How Does the Sun Angle Sensor Impact Learning?}

% Including the Sun Angle Sensor always decreases the total Delta V usage, which leads to an increased total reward. However, this more fuel-efficient behavior comes at the cost of fewer inspected points except when used with just the UPS.

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/sun_angle_effect/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/sun_angle_effect/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/sun_angle_effect/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/sun_angle_effect/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs. The top shows performance without the count sensor and the one below shows with the count sensor. This makes it easier to see the direct impact of adding the sensor.}
    \label{fig:impact_sun_angle}
\end{figure}

% When we look at the sample complexity plots, and focus on the inspected points (shown below), we see that including the sun angle sensor helps agents inspect more points early in training, but the benefit quickly collapses in favor of saving fuel. This is shown in the figure below. On the left, we have reward consistently increasing while on the right the number of inspected points starts to decrease. The top row shows all configurations and in the bottom row, we have extracted just the \textit{Sun Angle + Count} configuration to highlight the trend since it is the most drastic.

\begin{figure}
    \centering
    \subfigure[Total Reward with all sun angle configurations]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/only_sun_angle_agents/TotalReward_sample_eff.png}} \quad
    \subfigure[Inspected Points with all sun angle configurations]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/only_sun_angle_agents/InspectedPoints_sample_eff.png}} \\
    \subfigure[Total Reward only Sun Angle + Count]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/sun_angle_count/TotalReward_sample_eff.png}} \quad
    \subfigure[Inspected Points only Sun Angle + Count]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/sun_angle_count/InspectedPoints_sample_eff.png}} \\
    \subfigure[Legend for all sun angle configurations]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/only_sun_angle_agents/legend.png}}
    \caption{Top shows the sample complexity for Total Reward and Inspected Points for all configuration with the sun angle sensor (the legend is the bottom left). Bottom shows the sample complexity for just the Sun Angle + Count configuration to highlight the effect.}
    \label{fig:something_idk}
\end{figure}

% This behavior points towards the outsized cost of fuel for this problem. During training, we use a reward schedule that increases the cost of fuel for agents that have learned to inspect more than 90\% of points. The cost decreases when the agents start to inspect fewer than 80\% of points. This was intended to help the agent first focus on inspecting points and then finding the most fuel efficient policy for completing inspection. In the future we should consider investigating the impact of starting training with a more fuel efficient solution (e.g. already on a natural motion trajectory) as that might help find minimal adjustments needed to still inspect all points even with a moving chief.

\subsubsection{How Does the Uninspected Points Sensor Impact Learning?}

% Including the UPS always decreases the total Delta V usage and (except when added with the just the count sensor) always decreases the episode length. Unlike with the sun angle sensor, using the UPS to decrease fuel usage does not come at the cost of inspecting fewer points and increasing the episode length. Additionally, the number of points inspected increases and the majority of agents converge on policies that inspect all points. The only configurations where learned policies converge at a success rate higher than 75\% make use of the UPS. Without the UPS, agents rarely learn to inspect all the points more than 60\% of the time.

\begin{figure}
    \centering
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/ups_effect/TotalReward_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/ups_effect/Success_int_est.png}} \\
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/ups_effect/InspectedPoints_int_est.png}} \quad
    \subfigure[]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/ups_effect/DeltaV_int_est.png}}
    \caption{Final policy performance plots showing the expected level of performance of the final trained models. The line represents the interquartile mean and the shaded region is the 95\% confidence interval. The figures are structured to present the configurations in pairs. The top shows performance without the count sensor and the one below shows with the count sensor. This makes it easier to see the direct impact of adding the sensor.}
    \label{fig:impact_ups}
\end{figure}

% To highlight the impact of the UPS on helping agents inspect all 99 inspection points, we present the done conditions for the final policies trained with and without the UPS below. On the left are the done conditions reported for all 10 RL agents trained using a configuration without the UPS. On the right are the reported done conditions for all 10 RL agents trained using a configuration with the UPS. In both cases illustrated below, we see a large jump in the percentage of done conditions that show `SuccessfulInspection`.

\begin{figure}
    \centering
    \subfigure[AllButUPS]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/final_dones/count_sun_angle_final_policy_done.png}} \quad
    \subfigure[WithUPS]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/final_dones/baseline_final_policy_done.png}} \\
    \caption{The done conditions for all the learned policies looking at `All Sensors - UPS` on the left and `All Sensors` on the right. The increase in successful inspections from 26.7\% to 47.5\% shows more agents learning to converge to successful behavior.}
    \label{fig:impact_ups}
\end{figure}

\begin{figure}
    \centering
    \subfigure[count]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/final_dones/count_final_policy_done.png}} \quad
    \subfigure[countUPS]{\includegraphics[width=.45\linewidth]{figures/discrete/different_obs_spaces/final_dones/count_uninspected_final_policy_done.png}} \\
    \caption{The done conditions for all the learned policies looking at `Count` on the left and `Count + UPS` on the right. The increase in successful inspections from 33.4\% to 49.6\% shows more agent al learning to converge to successful behavior.}
    \label{fig:impact_ups}
\end{figure}

\subsection{Tables}


% \begin{table}[]
% \centering
% \caption{Table of InterQuartile Means and 95\% CI}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{lllllll}
% \toprule
% Metric Labels &             Total Reward &         Inspected Points &                Episode Length &          Success Rate &                     Delta V & Safety Violation Percentage \\
% \midrule
% No Sensors             &    8.001 [7.934, 8.0657] &  98.738 [98.564, 98.858] &  605.986 [579.7618, 633.7781] &   0.828 [0.776, 0.88] &   13.6232 [13.137, 14.1132] &    9.6044 [9.0212, 10.2067] \\
% Count                  &  3.2623 [3.2213, 3.3022] &  90.084 [89.502, 90.634] &    275.158 [272.028, 278.252] &   0.044 [0.008, 0.08] &  56.2937 [55.5938, 56.9782] &  16.1388 [15.8468, 16.4369] \\
% Sun Angle              &   7.5459 [7.4405, 7.647] &  90.942 [89.674, 92.082] &  852.876 [813.1899, 891.3521] &  0.162 [0.108, 0.216] &      8.2007 [7.691, 8.7292] &  11.4012 [10.8437, 11.9774] \\
% UPS                    &  8.2142 [8.1286, 8.2948] &  96.342 [95.308, 97.184] &   346.368 [335.5799, 356.832] &   0.584 [0.526, 0.64] &       9.459 [9.1485, 9.791] &   10.705 [10.1501, 11.2867] \\
% Count and Sun Angle    &  3.2215 [3.1806, 3.2617] &  85.838 [85.276, 86.386] &    254.038 [250.814, 257.292] &        0.0 [0.0, 0.0] &  52.7952 [52.0397, 53.5363] &  14.9818 [14.6266, 15.3396] \\
% Count and UPS          &   8.697 [8.6073, 8.7833] &   92.382 [91.412, 93.31] &    279.728 [273.404, 285.842] &   0.28 [0.226, 0.334] &      4.784 [4.6857, 4.8857] &   11.095 [10.3898, 11.8325] \\
% Sun Angle and UPS      &  9.3177 [9.2713, 9.3566] &   98.26 [97.836, 98.554] &     342.37 [337.06, 347.9221] &  0.706 [0.648, 0.764] &       3.229 [3.114, 3.3492] &     0.4742 [0.3274, 0.6381] \\
% All Sensors (baseline) &    8.98 [8.9175, 9.0345] &  96.764 [96.108, 97.314] &    334.93 [327.122, 342.7881] &   0.476 [0.422, 0.53] &      5.1842 [5.0273, 5.345] &     2.8884 [2.4858, 3.3471] \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[]
\centering
\caption{Table of InterQuartile Means and Standard Deviations}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lllllll}
\toprule
Metric Labels &          TotalReward &      InspectedPoints &           EpisodeLength &             Success &                DeltaV &                Safety \\
\midrule
No Sensors             &   7.9979 $\pm$ 0.417 &  98.732 $\pm$ 0.6604 &  604.808 $\pm$ 173.9998 &  0.826 $\pm$ 0.3791 &  13.5972 $\pm$ 3.6895 &   9.5735 $\pm$ 4.4831 \\
Count                  &  3.2602 $\pm$ 0.2864 &   90.05 $\pm$ 5.1919 &    274.96 $\pm$ 29.1013 &  0.042 $\pm$ 0.2006 &   56.2498 $\pm$ 6.324 &   16.1128 $\pm$ 3.878 \\
Sun Angle              &  7.5416 $\pm$ 0.6223 &  90.896 $\pm$ 7.3352 &  851.258 $\pm$ 282.0017 &   0.16 $\pm$ 0.3666 &    8.176 $\pm$ 3.3751 &   11.3775 $\pm$ 3.423 \\
UPS                    &  8.2107 $\pm$ 0.4757 &  96.304 $\pm$ 4.8452 &    345.88 $\pm$ 57.1779 &  0.582 $\pm$ 0.4932 &   9.4453 $\pm$ 1.8361 &   10.681 $\pm$ 3.3117 \\
Count and Sun Angle    &  3.2193 $\pm$ 0.2983 &   85.81 $\pm$ 3.9413 &   253.864 $\pm$ 25.4351 &       0.0 $\pm$ 0.0 &  52.7527 $\pm$ 6.2112 &  14.9673 $\pm$ 2.0386 \\
Count and UPS          &  8.6933 $\pm$ 0.5897 &  92.344 $\pm$ 6.6596 &   279.464 $\pm$ 40.6086 &   0.278 $\pm$ 0.448 &    4.7797 $\pm$ 0.592 &  11.0665 $\pm$ 4.2203 \\
Sun Angle and UPS      &   9.316 $\pm$ 0.2172 &  98.246 $\pm$ 1.5341 &   342.132 $\pm$ 31.2994 &  0.704 $\pm$ 0.4565 &   3.2237 $\pm$ 0.7442 &   0.4682 $\pm$ 0.8636 \\
All Sensors (baseline) &  8.9773 $\pm$ 0.3347 &   96.736 $\pm$ 3.395 &   334.572 $\pm$ 42.9696 &  0.474 $\pm$ 0.4993 &   5.1775 $\pm$ 0.9472 &   2.8714 $\pm$ 2.3382 \\
\bottomrule
\end{tabular}
}
\end{table}


% \begin{table}[]
% \centering
% \caption{Table of Means and 95\% CI}
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{lllllll}
% \toprule
% Metric Labels &             Total Reward &         Inspected Points &               Episode Length &          Success Rate &                     Delta V & Safety Violation Percentage \\
% \midrule
% No Sensors             &  7.6055 [7.5041, 7.7038] &  92.014 [90.988, 92.993] &  669.499 [649.7939, 689.402] &   0.664 [0.638, 0.69] &  14.7989 [14.3192, 15.2914] &  12.3548 [11.6805, 13.0598] \\
% Count                  &  3.1643 [3.0658, 3.2547] &  86.693 [85.815, 87.526] &    280.371 [274.76, 286.253] &   0.272 [0.254, 0.29] &  54.6395 [53.5217, 55.8079] &  16.8697 [16.3475, 17.4321] \\
% Sun Angle              &   6.9939 [6.8592, 7.127] &  82.941 [81.581, 84.282] &  780.048 [755.4758, 804.186] &  0.331 [0.304, 0.358] &    11.4816 [10.8525, 12.12] &  14.9469 [14.1322, 15.7812] \\
% UPS                    &  7.9007 [7.8177, 7.9811] &  89.781 [88.924, 90.607] &  398.068 [383.5039, 412.933] &   0.542 [0.513, 0.57] &  10.3844 [10.0608, 10.7112] &  12.8303 [12.1998, 13.4777] \\
% Count and Sun Angle    &  3.1169 [3.0729, 3.1597] &  83.719 [82.824, 84.572] &  248.921 [245.023, 252.6881] &  0.124 [0.107, 0.141] &  52.1599 [51.3116, 52.9747] &  16.6114 [15.9874, 17.2637] \\
% Count and UPS          &  8.4226 [8.3602, 8.4848] &  89.134 [88.506, 89.754] &   288.976 [281.652, 296.658] &   0.39 [0.363, 0.417] &     4.8775 [4.7817, 4.9739] &  12.2191 [11.6564, 12.7875] \\
% Sun Angle and UPS      &  8.8742 [8.7909, 8.9516] &  92.736 [91.958, 93.476] &   378.096 [367.34, 389.1912] &  0.603 [0.574, 0.632] &     3.7439 [3.6084, 3.8831] &     3.4146 [2.9255, 3.9305] \\
% All Sensors (baseline) &  8.5558 [8.4886, 8.6209] &   91.14 [90.478, 91.789] &  366.606 [354.7719, 378.762] &  0.488 [0.461, 0.515] &     5.4916 [5.3398, 5.6459] &      7.1023 [6.409, 7.8188] \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[]
\centering
\caption{Table of Means and Standard Deviations}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lllllll}
\toprule
Metric Labels &          TotalReward &       InspectedPoints &           EpisodeLength &             Success &                 DeltaV &                 Safety \\
\midrule
No Sensors             &  7.6055 $\pm$ 1.7189 &  92.014 $\pm$ 16.7788 &  669.499 $\pm$ 356.0666 &  0.664 $\pm$ 0.4723 &  14.7989 $\pm$ 10.5335 &   12.3548 $\pm$ 12.678 \\
Count                  &  3.1643 $\pm$ 1.7656 &  86.693 $\pm$ 15.8072 &   280.371 $\pm$ 114.278 &   0.272 $\pm$ 0.445 &  54.6395 $\pm$ 23.8811 &  16.8697 $\pm$ 11.0444 \\
Sun Angle              &  6.9939 $\pm$ 2.2902 &   82.941 $\pm$ 22.003 &  780.048 $\pm$ 428.7377 &  0.331 $\pm$ 0.4706 &  11.4816 $\pm$ 11.8938 &  14.9469 $\pm$ 14.0257 \\
UPS                    &  7.9007 $\pm$ 1.3483 &  89.781 $\pm$ 14.4545 &  398.068 $\pm$ 259.3268 &  0.542 $\pm$ 0.4982 &   10.3844 $\pm$ 5.5697 &  12.8303 $\pm$ 10.8549 \\
Count and Sun Angle    &  3.1169 $\pm$ 0.8576 &   83.719 $\pm$ 15.305 &   248.921 $\pm$ 73.2775 &  0.124 $\pm$ 0.3296 &  52.1599 $\pm$ 16.9304 &  16.6114 $\pm$ 10.3814 \\
Count and UPS          &  8.4226 $\pm$ 1.1149 &  89.134 $\pm$ 11.2445 &  288.976 $\pm$ 129.2508 &   0.39 $\pm$ 0.4877 &    4.8775 $\pm$ 1.6782 &   12.2191 $\pm$ 9.2755 \\
Sun Angle and UPS      &  8.8742 $\pm$ 1.3319 &  92.736 $\pm$ 12.7588 &  378.096 $\pm$ 192.5143 &  0.603 $\pm$ 0.4893 &    3.7439 $\pm$ 2.4747 &    3.4146 $\pm$ 8.3665 \\
All Sensors (baseline) &  8.5558 $\pm$ 1.1968 &   91.14 $\pm$ 12.1686 &  366.606 $\pm$ 208.7727 &  0.488 $\pm$ 0.4999 &    5.4916 $\pm$ 2.6249 &   7.1023 $\pm$ 11.6083 \\
\bottomrule
\end{tabular}
}
\end{table}
